Countering Racial Bias in Computer Graphics Research

Current computer graphics research practices contain racial biases that have resulted in investigations into "skin" and "hair" that focus on the hegemonic visual features of Europeans and East Asians. To broaden our research horizons to encompass all of humanity, we propose a variety of improvements to quantitative measures and qualitative practices, and pose novel, open research problems.

==> commenting-macros.tex <==
% !TEX root = unbiased.tex
% Set the comment type
% 0 - comments disabled
% 1 - inline comments
% 2 - PDF comments
% 3 - margin comments
\def\commentType{1}

\usepackage{xargs}


% Comments
\ifnum\commentType=0
    % This causes double spaces when comments are written with spaces around them in the middle of a sentence.
    % For example, "This is \Peter{This is a comment.} a sentence." renders as "This is  a sentence.".
    % TODO: Fix this.
    \newcommandx{\customComment}[3]{}
    \newcommandx{\customTODO}[3]{}
\fi
\ifnum\commentType=1
    % \usepackage[
    % type=upperleft,
    % unit=in
    % ]{fgruler}
    \newcommandx{\customComment}[3]{{\small\textcolor{#2}{[\textsl{#1: #3}]}}}
    \newcommandx{\customTODO}[3]{{\small\textcolor{#2}{[\textsl{#1: #3}]}}}
\fi
\ifnum\commentType=2
    % \usepackage[
    % type=upperleft,
    % unit=in
    % ]{fgruler}
    \usepackage{pdfcomment}
    \newcommandx{\customComment}[3]{\pdfcomment[icon=Comment,opacity=0.5,color=#2,author=#1]{#3}}
    \newcommandx{\customTODO}[3]{\pdfcomment[icon=Note,opacity=0.5,color=#2,author=#1]{#3}}
\fi
\ifnum\commentType=3
    \usepackage[
    type=upperleft,
    unit=in
    ]{fgruler}
    % \usepackage{pdfcomment} % somehow this helps avoiding an error
    \addtolength{\paperwidth}{2in}
    \addtolength{\oddsidemargin}{1in}
    \addtolength{\evensidemargin}{1in}
    \setlength{\marginparwidth}{1.5in}
    \setlength{\marginparsep}{.1in}
    \usepackage{todonotes} % Use [disable] argument to disable todonotes.
    % Silence warnings that todonotes package occasionally generates
    % \usepackage{silence}
    % \WarningFilter*{latex}{Marginpar on page \thepage\space moved}
    \newcommandx{\customComment}[3]{\todo[color=#2!40,size=\small]{\textbf{#1:} #3}}
    \newcommandx{\customTODO}[3]{\todo[color=#2!40,size=\small]{\textbf{#1:} #3}}
\fi

\definecolor{jade}{HTML}{00d2d3}
\definecolor{ultraviolet}{HTML}{5f27cd}
\definecolor{heliotrope}{HTML}{e056fd}
\definecolor{shamrock}{HTML}{10ac84}
\definecolor{love}{HTML}{ee5253}
\definecolor{dragon}{HTML}{ff9f43}

% for work in progress
\newcommandx{\REMOVE}[1]{{\color{love}\st{#1}}} 
\newcommandx{\ADD}[1]{{\textcolor{shamrock}{#1}}}

 % for final version
%\newcommandx{\REMOVE}[1]{}
%\newcommandx{\ADD}[1]{#1}

\newcommandx{\TODO}[1]{\customComment{TODO}{heliotrope}{#1}}
\newcommandx{\TK}[1]{\customComment{Ted}{jade}{#1}}
\newcommandx{\JD}[1]{\customComment{Julie}{heliotrope}{#1}}
\newcommandx{\HR}[1]{\customComment{Holly}{shamrock}{#1}}
\newcommandx{\DN}[1]{\customComment{Derek}{dragon}{#1}}
\newcommandx{\WJ}[1]{\customComment{Wojtek}{jade}{#1}}
\newcommandx{\AM}[1]{\customComment{A.M.}{love}{#1}}
